RAIST: Learning Risk Aware Traffic Interactions via Spatio-Temporal Graph Convolutional Networks

A key aspect of driving a road vehicle is to interact with other road users, assess their intentions and make risk-aware tactical decisions. An intuitive approach to enabling an intelligent automated driving system would be incorporating some aspects of human driving behavior. To this end, we propose a novel driving framework for egocentric views based on spatio-temporal traffic graphs. The traffic graphs model not only the spatial interactions amongst the road users but also their individual intentions through temporally associated message passing. We leverage a spatio-temporal graph convolutional network (ST-GCN) to train the graph edges. These edges are formulated using parameterized functions of 3D positions and scene-aware appearance features of road agents. Along with tactical behavior prediction, it is crucial to evaluate the risk-assessing ability of the proposed framework. We claim that our framework learns risk-aware representations by improving on the task of risk object identification, especially in identifying objects with vulnerable interactions like pedestrians and cyclists.

==> sections/abstract.tex <==
\begin{abstract}

A key aspect of driving a road vehicle is to interact with the other road users, assess their intentions and make risk-aware tactical decisions. An intuitive approach of enabling an intelligent automated driving system would be to incorporate some aspects of the human driving behavior. To this end, we propose a novel driving framework for egocentric views, which is based on spatio-temporal traffic graphs. The traffic graphs not only model the spatial interactions amongst the road agents, but also their individual intentions through temporally associated message passing. We leverage spatio-temporal graph convolutional network (ST-GCN) to train the graph edges. These edges are formulated using parameterized functions of 3D positions and scene-aware appearance features of road agents. Along with tactical behavior prediction, it is crucial to evaluate the risk assessing ability of the proposed framework. We claim that our framework can learn risk aware representations by improving on the task of risk object identification, especially in identifying objects with vulnerable interactions like pedestrians and cyclists.

\end{abstract}
